Differentially Private Computation of Basic Reproduction Numbers in Networked Epidemic Models

The basic reproduction number of a networked epidemic model, denoted $R_0$, can be computed from a network's topology to quantify epidemic spread. However, disclosure of $R_0$ risks revealing sensitive information about the underlying network, such as an individual's relationships within a social network. Therefore, we propose a framework to compute and release $R_0$ in a differentially private way. First, we provide a new result that shows how $R_0$ can be used to bound the level of penetration of an epidemic within a single community as a motivation for the need of privacy, which may also be of independent interest. We next develop a privacy mechanism to formally safeguard the edge weights in the underlying network when computing $R_0$. Then we formalize tradeoffs between the level of privacy and the accuracy of values of the privatized $R_0$. To show the utility of the private $R_0$ in practice, we use it to bound this level of penetration under privacy, and concentration bounds on these analyses show they remain accurate with privacy implemented. We apply our results to real travel data gathered during the spread of COVID-19, and we show that, under real-world conditions, we can compute $R_0$ in a differentially private way while incurring errors as low as $7.6\%$ on average.

==> Accuracy_undirected_graph.tex <==
\section{Generating Differentially Private Basic Reproduction Number for Directed Graphs}\label{sec:directed_graphs}

In the previous section, we defined the differential privacy mechanisms for the basic reproduction number in the undirected graph. In this section, we extend the input mechanism defined in Mechanism~\ref{mech:bounded_Gaussian_mechanism} to the directed graphs.

\begin{mechanism}[Bounded Gaussian mechanism]\label{mech:bounded_Gaussian_mechanism_directed}
Fix a probability space $(\Omega,\mathcal{F},\mathbb{P})$. Let $\sigma>0$ and let $G=(V,E,W)$ be the sensitive graph. Then for $D=(0,\bar{w}]$, the bounded Gaussian mechanism $M_{BG}:D^{n_w}\times \Omega \rightarrow D^{n_w}$ generates independent private weights $\Tilde{w}_{ij}\sim \text{TrunG}(w_{ij},\sigma,0,\Bar{w})$.
The minimal $\sigma=\Omega\left(\sqrt{\frac{2\Bar{w}\Delta_2w+(\Delta_2w)^2}{\epsilon}}\right)$ that satisfies $\epsilon$-differential privacy can be found using \cite[Algorithm 2]{chen2022bounded} by setting $\Delta_2w= k$. \bo{Here we will add independent noise to all entries in matrix $W$.}\hfill $\lozenge$
\end{mechanism}

The accuracy of Mechanism~\ref{mech:bounded_Gaussian_mechanism_directed} can be quantified by a modified version of Theorem~\ref{thm:expectation_bound_input_perturb}.

\begin{thm}\label{thm:expectation_bound_input_perturb_directed}
    Let $\alpha_{ij}=\frac{-w_{ij}}{\sigma}$ and $\beta_{ij}=\frac{\Bar{w}-w_{ij}}{\sigma}$. Given a sensitive \bo{directed} graph $G=(V,E,W)$ with its reproduction number $R_0=\rho(W)$, for private graphs $\Tilde{G}=(V,E,\Tilde{W})$, whose weights $\Tilde{W}=M_{BG}(W)$ is generated by the bounded Gaussian mechanism with privacy parameter $\epsilon$ and the private reproduction number $\Tilde{R}_0=\rho(\Tilde{W})$, we have
    \begin{align}
        \mathbb{E}[\Tilde{R}_0-R_0]&\leq\mathbb{E}[|\Tilde{R}_0-R_0|]\leq \sigma \cdot \Xi+\kappa\leq \sigma\sqrt{n_w}+\kappa,\label{eq:abs_expectation_bounds_input_perturb_directed}
    \end{align}
    and
    \begin{align}
        &\mathbb{E}[(\Tilde{R}_0-R_0)^2]\leq (\sigma \cdot \Xi+\kappa)^2\leq (\sigma\sqrt{n_w}+\kappa)^2\label{eq:mse_bounds_input_perturb_directed},
    \end{align}
    where
    \begin{align}
        \Xi &= \sqrt{n_w-\sum_{i=1}^n\sum_{j=1}^n\frac{\beta_{ij}\varphi(\beta_{ij})-\alpha_{ij}\varphi(\alpha_{ij})}{\Phi(\beta_{ij})-\Phi(\alpha_{ij})}}\\
        \kappa &= ||W||_2 - R_0\label{eq:residual_error_directed}
    \end{align}
\end{thm}

\emph{Proof:} See Appendix~\ref{apdx:expectation_bound_input_perturb_directed}.\hfill $\blacksquare$

We next state a tail bound on the $\tilde{R}_0$ to bound deviation from this mean error.

\begin{thm}[Tail bounds]\label{thm:input_perturb_tail}
    Given a sensitive graph $G=(V,E,W)\in\mathcal{G}^n$ with its reproduction number $R_0=\rho(W)$, for private graphs $\tilde{G}=(V,E,\tilde{W})\in\mathcal{G}^n$ whose weights $\tilde{W}=M_{BG}(W)$ is generated by the bounded Gaussian mechanism with privacy parameter $\epsilon$ and private reproduction number $\tilde{R}_0=\rho(\tilde{W})$, we have
    \begin{equation}
        \tilde{R}_0 - R_0\leq \sigma\sqrt{n_w} + r + \kappa,
    \end{equation}
    where $\kappa$ is defined in Equation~\eqref{eq:residual_error_directed} and $r$ is a random variable that satisfies the tail bound:
    \begin{equation}
        \mathbb{P}[r>t]\leq C\cdot\exp\left(-\frac{t^2}{2\sigma^2}\right),
    \end{equation}
    where $C=2\cdot 9^{2n}$ and $\sigma$ is the minimal value from Mechanism~\ref{mech:bounded_Gaussian_mechanism} that is required for the bounded Gaussian mechanism to satisfy $\epsilon$-differential privacy.
\end{thm}
\emph{Proof:} See Appendix~\ref{apdx:proof_input_perturb_tail}.\hfill $\blacksquare$

\bo{Add a remark to say the huge constant $C$ is not a problem.}

==> CaseStudy.tex <==
\section{Simulations}\label{sec:casestudy}
In this section, we present simulation results, i.e., $\Tilde{R}_0$, generated by input and output perturbation. 
We start by considering random, connected, and undirected networks with $n=20$ nodes. 
%Moreover, in simulations we only allow bidirectional edges since in the context of epidemic networks for communities, \baike{ we assume disease transmission between communities is mutual with the same transmission rate.} %(\bo{Does this make sense? Maybe some references?})
We set the number of edges in these networks, denoted as $n_e$, equal to 100. The process of generating a random undirected network involves the following steps. 
First, we generate a uniformly chosen spanning tree using the random walk algorithm~\cite{Wilson1996Random}. 
Next, until the desired number of edges $n_e$ has been reached, we add an edge between any two uniformly chosen nodes. Then, we add self loops for all nodes.   
%Each undirected edge is then converted into a pair of directed edges, one in each direction. 
Lastly, weights are generated by uniformly chosen from the interval $(0,\Bar{w}]$ with $\Bar{w}=3$, i.e., $\gamma_{min}=\frac{1}{3}$, %(\bo{Does this number make sense?}), 
for all undirected edges. The adjacency parameter $k$ is set to 3 for all simulations.


\begin{figure}[t!]
    \centering
        % This file was created with tikzplotlib v0.9.12.
    % This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
width=\columnwidth, 
height=4cm,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\footnotesize Privacy Parameter \(\displaystyle \epsilon\)},
xmajorgrids,
xmin=0.65, xmax=10.55,
xtick style={color=black},
y grid style={darkgray176},
ylabel={\footnotesize Avg. of \(\displaystyle |\tilde{R}_0-R_0|\)},
ymajorgrids,
ymin=0.128076841502687, ymax=4.36488023934154,
ytick style={color=black}
]
\addplot [very thick, blue, mark=*, mark size=2, mark options={solid}]
table {%
1.1 4.17229826671251
2.1 1.95758641330742
3.1 1.22800866375149
4.1 0.871000829475826
5.1 0.683499436117528
6.1 0.554902535252702
7.1 0.466924972120081
8.1 0.404634494063549
9.1 0.353741620983036
10.1 0.320658814131726
};
\addlegendentry{Input Pertubation}
\addplot [very thick, red, mark=*, mark size=2, mark options={solid}]
table {%
1.1 0.954358546509518
2.1 0.969250864194753
3.1 0.963484725610941
4.1 0.959582514114931
5.1 0.959944679831626
6.1 0.953447412447068
7.1 0.954320368457293
8.1 0.949455472707502
9.1 0.952947968967866
10.1 0.937352424027365
};
\addlegendentry{Output Pertubation}
\end{axis}

\end{tikzpicture}



    \caption{Empirical average of $|\tilde{R}_0-R_0|$ as a function of privacy parameter $\epsilon$. Smaller values of the level of privacy $\epsilon$
    correspond to a stronger level of privacy.}
    \label{fig:abs_avg_acc_loss_vs_epsilon}
\end{figure}

\begin{figure}[t!]
    \centering
    % This file was created with tikzplotlib v0.10.1.
    \begin{tikzpicture}
    
    \definecolor{darkgray176}{RGB}{176,176,176}
    \definecolor{darkorange25512714}{RGB}{255,127,14}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{steelblue31119180}{RGB}{31,119,180}
    
    \begin{axis}[
    width=\columnwidth, 
    height=4.5cm,
    legend cell align={left},
    legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204, font=\fontsize{9}{5}\selectfont},
    tick align=outside,
    tick pos=left,
    x grid style={darkgray176},
    xlabel={\footnotesize Value of Private Results \(\displaystyle \tilde{R}_0\)},
    xmin=-2, xmax=42,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel={\footnotesize Counts},
    ymin=0, ymax=583.8,
    ytick style={color=black}
    ]
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:0,0) rectangle (axis cs:1.37931034482759,6);
    \addlegendimage{ybar,ybar legend,draw=none,fill=steelblue31119180,fill opacity=0.75}
    \addlegendentry{Output Perturbation}
    
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:1.37931034482759,0) rectangle (axis cs:2.75862068965517,3);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:2.75862068965517,0) rectangle (axis cs:4.13793103448276,9);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:4.13793103448276,0) rectangle (axis cs:5.51724137931034,12);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:5.51724137931035,0) rectangle (axis cs:6.89655172413793,10);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:6.89655172413793,0) rectangle (axis cs:8.27586206896552,19);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:8.27586206896552,0) rectangle (axis cs:9.6551724137931,21);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:9.6551724137931,0) rectangle (axis cs:11.0344827586207,28);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:11.0344827586207,0) rectangle (axis cs:12.4137931034483,54);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:12.4137931034483,0) rectangle (axis cs:13.7931034482759,47);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:13.7931034482759,0) rectangle (axis cs:15.1724137931034,84);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:15.1724137931034,0) rectangle (axis cs:16.551724137931,112);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:16.551724137931,0) rectangle (axis cs:17.9310344827586,152);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:17.9310344827586,0) rectangle (axis cs:19.3103448275862,120);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:19.3103448275862,0) rectangle (axis cs:20.6896551724138,84);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:20.6896551724138,0) rectangle (axis cs:22.0689655172414,59);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:22.0689655172414,0) rectangle (axis cs:23.448275862069,50);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:23.448275862069,0) rectangle (axis cs:24.8275862068966,34);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:24.8275862068966,0) rectangle (axis cs:26.2068965517241,24);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:26.2068965517241,0) rectangle (axis cs:27.5862068965517,28);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:27.5862068965517,0) rectangle (axis cs:28.9655172413793,17);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:28.9655172413793,0) rectangle (axis cs:30.3448275862069,4);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:30.3448275862069,0) rectangle (axis cs:31.7241379310345,5);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:31.7241379310345,0) rectangle (axis cs:33.1034482758621,6);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:33.1034482758621,0) rectangle (axis cs:34.4827586206897,1);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:34.4827586206897,0) rectangle (axis cs:35.8620689655172,4);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:35.8620689655172,0) rectangle (axis cs:37.2413793103448,1);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:37.2413793103448,0) rectangle (axis cs:38.6206896551724,2);
    \draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:38.6206896551724,0) rectangle (axis cs:40,1);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:0,0) rectangle (axis cs:1.37931034482759,0);
    \addlegendimage{ybar,ybar legend,draw=none,fill=darkorange25512714,fill opacity=0.5}
    \addlegendentry{Input Perturbation}
    
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:1.37931034482759,0) rectangle (axis cs:2.75862068965517,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:2.75862068965517,0) rectangle (axis cs:4.13793103448276,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:4.13793103448276,0) rectangle (axis cs:5.51724137931034,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:5.51724137931035,0) rectangle (axis cs:6.89655172413793,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:6.89655172413793,0) rectangle (axis cs:8.27586206896552,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:8.27586206896552,0) rectangle (axis cs:9.6551724137931,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:9.6551724137931,0) rectangle (axis cs:11.0344827586207,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:11.0344827586207,0) rectangle (axis cs:12.4137931034483,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:12.4137931034483,0) rectangle (axis cs:13.7931034482759,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:13.7931034482759,0) rectangle (axis cs:15.1724137931034,5);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:15.1724137931034,0) rectangle (axis cs:16.551724137931,137);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:16.551724137931,0) rectangle (axis cs:17.9310344827586,556);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:17.9310344827586,0) rectangle (axis cs:19.3103448275862,280);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:19.3103448275862,0) rectangle (axis cs:20.6896551724138,22);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:20.6896551724138,0) rectangle (axis cs:22.0689655172414,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:22.0689655172414,0) rectangle (axis cs:23.448275862069,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:23.448275862069,0) rectangle (axis cs:24.8275862068966,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:24.8275862068966,0) rectangle (axis cs:26.2068965517241,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:26.2068965517241,0) rectangle (axis cs:27.5862068965517,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:27.5862068965517,0) rectangle (axis cs:28.9655172413793,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:28.9655172413793,0) rectangle (axis cs:30.3448275862069,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:30.3448275862069,0) rectangle (axis cs:31.7241379310345,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:31.7241379310345,0) rectangle (axis cs:33.1034482758621,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:33.1034482758621,0) rectangle (axis cs:34.4827586206897,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:34.4827586206897,0) rectangle (axis cs:35.8620689655172,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:35.8620689655172,0) rectangle (axis cs:37.2413793103448,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:37.2413793103448,0) rectangle (axis cs:38.6206896551724,0);
    \draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:38.6206896551724,0) rectangle (axis cs:40,0);
    \addplot [semithick, red, dashed]
    table {%
    17.4365656267109 -1.4210854715202e-14
    17.4365656267109 583.8
    };
    \addlegendentry{$R_0=17.44$}
    \end{axis}
    
    \end{tikzpicture}

    \caption{A histogram of private results $\tilde{R}_0$ for one graph when the level of privacy $\epsilon=1$. The samples generated by input perturbation (orange rectangles) are more concentrated around the true value (red dashed line) compared to output perturbation (blue rectangles).}
    \label{fig:private_samples_compare_epsilon_1}
\end{figure}

\begin{figure}[t!]
    \centering
    % This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
width=\columnwidth, 
height=4.5cm,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204, font=\fontsize{7}{5}\selectfont},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\footnotesize Value of Private Results \(\displaystyle \tilde{R}_0\)},
xmin=13.65, xmax=21.35,
xtick style={color=black},
y grid style={darkgray176},
ylabel={\footnotesize Counts},
ymin=0, ymax=235.2,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:14,0) rectangle (axis cs:14.2413793103448,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=steelblue31119180,fill opacity=0.75}
\addlegendentry{Output Perturbation}

\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:14.2413793103448,0) rectangle (axis cs:14.4827586206897,1);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:14.4827586206897,0) rectangle (axis cs:14.7241379310345,1);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:14.7241379310345,0) rectangle (axis cs:14.9655172413793,1);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:14.9655172413793,0) rectangle (axis cs:15.2068965517241,3);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:15.2068965517241,0) rectangle (axis cs:15.448275862069,3);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:15.448275862069,0) rectangle (axis cs:15.6896551724138,3);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:15.6896551724138,0) rectangle (axis cs:15.9310344827586,9);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:15.9310344827586,0) rectangle (axis cs:16.1724137931035,11);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:16.1724137931035,0) rectangle (axis cs:16.4137931034483,18);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:16.4137931034483,0) rectangle (axis cs:16.6551724137931,31);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:16.6551724137931,0) rectangle (axis cs:16.8965517241379,69);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:16.8965517241379,0) rectangle (axis cs:17.1379310344828,107);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:17.1379310344828,0) rectangle (axis cs:17.3793103448276,172);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:17.3793103448276,0) rectangle (axis cs:17.6206896551724,224);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:17.6206896551724,0) rectangle (axis cs:17.8620689655172,155);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:17.8620689655172,0) rectangle (axis cs:18.1034482758621,83);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:18.1034482758621,0) rectangle (axis cs:18.3448275862069,47);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:18.3448275862069,0) rectangle (axis cs:18.5862068965517,20);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:18.5862068965517,0) rectangle (axis cs:18.8275862068966,16);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:18.8275862068966,0) rectangle (axis cs:19.0689655172414,8);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:19.0689655172414,0) rectangle (axis cs:19.3103448275862,9);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:19.3103448275862,0) rectangle (axis cs:19.551724137931,4);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:19.551724137931,0) rectangle (axis cs:19.7931034482759,2);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:19.7931034482759,0) rectangle (axis cs:20.0344827586207,1);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:20.0344827586207,0) rectangle (axis cs:20.2758620689655,1);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:20.2758620689655,0) rectangle (axis cs:20.5172413793103,1);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:20.5172413793103,0) rectangle (axis cs:20.7586206896552,0);
\draw[draw=none,fill=steelblue31119180,fill opacity=0.75] (axis cs:20.7586206896552,0) rectangle (axis cs:21,0);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:14,0) rectangle (axis cs:14.2413793103448,0);
\addlegendimage{ybar,ybar legend,draw=none,fill=darkorange25512714,fill opacity=0.5}
\addlegendentry{Input Perturbation}

\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:14.2413793103448,0) rectangle (axis cs:14.4827586206897,1);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:14.4827586206897,0) rectangle (axis cs:14.7241379310345,1);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:14.7241379310345,0) rectangle (axis cs:14.9655172413793,3);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:14.9655172413793,0) rectangle (axis cs:15.2068965517241,3);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:15.2068965517241,0) rectangle (axis cs:15.448275862069,4);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:15.448275862069,0) rectangle (axis cs:15.6896551724138,12);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:15.6896551724138,0) rectangle (axis cs:15.9310344827586,29);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:15.9310344827586,0) rectangle (axis cs:16.1724137931035,39);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:16.1724137931035,0) rectangle (axis cs:16.4137931034483,41);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:16.4137931034483,0) rectangle (axis cs:16.6551724137931,62);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:16.6551724137931,0) rectangle (axis cs:16.8965517241379,78);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:16.8965517241379,0) rectangle (axis cs:17.1379310344828,97);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:17.1379310344828,0) rectangle (axis cs:17.3793103448276,119);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:17.3793103448276,0) rectangle (axis cs:17.6206896551724,101);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:17.6206896551724,0) rectangle (axis cs:17.8620689655172,105);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:17.8620689655172,0) rectangle (axis cs:18.1034482758621,81);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:18.1034482758621,0) rectangle (axis cs:18.3448275862069,74);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:18.3448275862069,0) rectangle (axis cs:18.5862068965517,47);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:18.5862068965517,0) rectangle (axis cs:18.8275862068966,44);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:18.8275862068966,0) rectangle (axis cs:19.0689655172414,20);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:19.0689655172414,0) rectangle (axis cs:19.3103448275862,21);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:19.3103448275862,0) rectangle (axis cs:19.551724137931,10);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:19.551724137931,0) rectangle (axis cs:19.7931034482759,7);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:19.7931034482759,0) rectangle (axis cs:20.0344827586207,1);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:20.0344827586207,0) rectangle (axis cs:20.2758620689655,0);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:20.2758620689655,0) rectangle (axis cs:20.5172413793103,0);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:20.5172413793103,0) rectangle (axis cs:20.7586206896552,0);
\draw[draw=none,fill=darkorange25512714,fill opacity=0.5] (axis cs:20.7586206896552,0) rectangle (axis cs:21,0);
\addplot [semithick, red, dashed]
table {%
17.4365656267109 -7.105427357601e-15
17.4365656267109 235.2
};
\addlegendentry{$R_0=17.44$}
\end{axis}

\end{tikzpicture}

    \caption{Histograms of private results $\tilde{R}_0$ for one graph when the level of privacy $\epsilon=7$. The one of input perturbation (orange rectangles) is flatter than output perturbation, which indicates a higher probability of getting noisy private results.}
    \label{fig:private_samples_compare_epsilon_7}
\end{figure}

In our simulations, we generated a total of 20 random undirected networks, along with 1000 private networks with perturbed weights $\Tilde{W}$ using the input perturbation mechanism in Mechanism~\ref{mech:bounded_Gaussian_mechanism} for each random network. Moreover, we generated a total of 1000 private basic reproduction numbers $\tilde{R}_0$ by the output perturbation mechanism in Mechanism~\ref{mech:bounded_laplace} for each of the randomly generated networks. 

\textbf{The input perturbation mechanism is more robust than the output perturbation mechanism in the high privacy regime.} 
Figure~\ref{fig:abs_avg_acc_loss_vs_epsilon} illustrates the effect of privacy on the accuracy of private reproduction numbers $\Tilde{R}_0$. We compute the empirical average over all random networks and all corresponding absolute differences $|\Tilde{R}_0-R_0|$ under input and output perturbation. When $\epsilon$ is close to 0, the output perturbation mechanism results in a much higher accuracy loss compared to the input perturbation mechanism. 
%Intuitively, fix other variables, according to Equation~\eqref{eq:mse_bounds_input_perturb} the expectation on the mean square error of the input perturbation is upper bounded by 
%\begin{equation}
%    E[(\Tilde{R}_0-R_0)^2]\leq n_w\sigma^2, \text{ where }\sigma^2=\Omega\left(\frac{1}{\epsilon}\right),\label{eq:mse_bounds_input_perturb_bigo}
%\end{equation}
%By contrast, applying~\eqref{eq:mse_bounds_output_perturb}, we have
%\begin{equation}
%    E[(\Tilde{R}_0-R_0)^2]\leq 2b_L^2, \text{ where } b_L^2=\Omega\left(\frac{1}{\epsilon^2}\right).\label{eq:mse_bounds_output_perturb_bigo}
%\end{equation}
Specifically, private results $\Tilde{R}_0$ generated by the output perturbation mechanism are more likely to be far away from the true value of $R_0$ when $\epsilon\rightarrow 0$. Indeed, in Figure~\ref{fig:private_samples_compare_epsilon_1}, we observe that the samples of $\Tilde{R}_0$ generated by the input perturbation mechanism are more concentrated compared to the output perturbation mechanism when $\epsilon=1$, which is small.

%$\epsilon$-differential privacy guarantee, the input perturbation mechanism requires a minimal parameter $\sigma=\mathcal{O}\left(\sqrt{\frac{1}{\epsilon}}\right)$ while the output perturbation mechanism requires a minimal parameter $b=\mathcal{O}\left(\frac{1}{\epsilon}\right)$
%Intuitively, this is because private $\Tilde{R}_0$ generated by the input perturbation is a bounded random variable with a smaller domain compared to the output perturbation. In high privacy regime, A histogram of samples of private $\tilde{R}_0$ when setting the privacy parameter $\epsilon=1$ is shown in 
%Figure~\ref{fig:private_samples_compare}. We observe that the samples of $\Tilde{R}_0$ generated by the input perturbation mechanism are more concentrated compared to the output perturbation mechanism.

By contrast, \textbf{the output perturbation mechanism outperforms the input perturbation mechanism in the low privacy regime.} Since higher values of privacy parameter $\epsilon$ imply weaker privacy, the simulation results in Figure~\ref{fig:abs_avg_acc_loss_vs_epsilon}confirm that weaker privacy guarantees result in smaller accuracy loss. However, we observe that while $\epsilon$ gets larger, the accuracy loss of output perturbation decreases much faster than the input perturbation, and eventually outperforms input perturbation. 
%This is confirmed by the Equation~\eqref{eq:mse_bounds_input_perturb_bigo},~\eqref{eq:mse_bounds_output_perturb_bigo}. 
An example of the empirical distributions of private samples with $\epsilon=7$ is shown in Figure~\ref{fig:private_samples_compare_epsilon_7}, which provides a strong empirical justification. We emphasize that even large $\epsilon$ provides stronger empirical privacy than no differential privacy guarantee.

==> Results.tex <==
\section{Private Epidemic Analysis}\label{sec:example_analysis}


%\colorbox{BurntOrange}{[add more discussion. Difference between $SIS$ and $SIR$.]}
%Theorem~\ref{thm_upper_bound} characterizes the susceptible proportion at a disease-free equilibrium within one community through the overall reproduction number of the network $R_0$. 
%Recall that the susceptible proportion within a community can capture the level of Penetration from a virus, i.e., the damage caused by the virus regard how many people are infected eventually during the spreading process. 
%Theorem~\ref{thm_upper_bound} indicates that, the reproduction number of the overall network $R_0$ can infer the further information within the community. Hence, it is critical to add privacy to the reproduction number of the overall network to protect unveiling further information of the spreading process within the community.



% \begin{thm}\label{thm:level_of_penetration_acc_bound_output_perturb}
%     Given a generalized graph $G=(V,E,W)$ where $R_0=\rho(W)$ and a privacy parameter $\epsilon$, for $t\in\left(0,\frac{1}{R_0}\right)$, the private reproduction number $\Tilde{R}_0$ generated by Mechanism~\ref{mech:bounded_laplace} satisfies
%     \begin{align}
%         &\mathbb{P}\left[\left|\frac{1}{\Tilde{R}_0}-\frac{1}{R_0}\right|<t\right]\\ 
%         &\qquad\qquad= \frac{\left(2-\exp\left(\frac{f(t)-R_0}{b_L}\right)-\exp\left(\frac{R_0-g(t)}{b_L}\right)\right)}{2C(R_0,b_L)},
%     \end{align}
%     where $f(t)=\frac{1}{\frac{1}{R_0}+t}$ and $g(t)=\frac{1}{\frac{1}{R_0}-t}$.
% \end{thm}
% \emph{Proof:} See Appendix~\ref{apdx:proof_level_of_penetration_acc_bound_output_perturb}\hfill $\blacksquare$

==> keywords.tex <==
\begin{IEEEkeywords}
	stuff
\end{IEEEkeywords}

==> privacy_mechanism_v1.tex <==
\section{Privacy mechanisms for the reproduction number}\label{sec:results}
In this section, we develop two distinct differentially private mechanisms that enforce differential privacy - one utilizing the input perturbation and the other employing the output perturbation. 

\subsection{Input Perturbation Mechanism}
The input perturbation mechanism provides differential privacy guarantee by generating private values for the weights of a graph. Specifically, we use the bounded Gaussian mechanism~\cite{chen2022bounded} for this purpose. We start by defining the sensitivity, which captures the maximum impact on outputs of changing a weighted graph $G=(V,E,w)$ (\bo{Unify the notations}) to an adjacent graph $G'=(V,E,w')$ in Definition~\ref{def:adjacency}.   

\begin{definition}[$L_2$ sensitivity]
Given an adjacency parameter $k$, then the $L_2$ sensitivity is defined as:
\begin{equation*}
    \Delta_2 w = \max_{\substack{G, G' \in \mathcal{G}_n \\ ||w(G)-w(G')||_1 \leq k}} \sqrt{\sum_{e\in E}(w(G)-w(G'))^2},
\end{equation*}
\end{definition}

Since the $L_2$ sensitivity is defined by $L_2$ norm of the vector-wise entries difference, by the nature of norms we have
\begin{equation}
    \Delta_2 w \leq k.
\end{equation}

We then use this upper bound on $\Delta_2w$ to calibrate the variance of noise needed to protect privacy. The private values are generated by the bounded Gaussian mechanism, whose outputs only lie in the interval $[\bm{0}^n,\bm{\Bar{w}}^n]$ \bo{Create a \emph{notations} paragraph and list this in. Assume $w\leq \Bar{w}$}. 

\begin{definition}[Bounded Gaussian mechanism; Solution to Problem~\ref{prob:input_perturbation_design}]
Fix a probability space $(\Omega,\mathcal{F},\mathbb{P})$. Let $\sigma>0$ and let $G=(V,E,w)$ be the sensitive graph. Then the bounded Gaussian mechanism $M_{BG}:[\bm{0}^n,\bm{\Bar{w}}^n]\times \Omega \rightarrow [\bm{0}^n,\bm{\bar{w}}^n]$ generates independent output for each entry $w_{ij}>0$ of $w(G)$ with the probability density function $p_{M_{BG}}$:
\begin{align}
    p_{M_{BG}}(x) = \begin{cases}
        \frac{1}{C_{w_{ij}}(\sigma)} \exp\left(-\frac{(x-w_{ij})^2}{2\sigma^2}\right) & \text{if } x\in (0, \Bar{w}] \\
        0 & \text{otherwise}
    \end{cases},
\end{align}
where $C_{w_{ij}}(\sigma)=\int_0^{\Bar{w}} \exp\left(-\frac{(x-w_{ij})^2}{2\sigma^2}\right)dx$ is the normalizing term. The minimal $\sigma>0$ that satisfies $(\epsilon,0)$-differential privacy can be found using Algorithm 2 in \cite{chen2022bounded} by setting $\Delta_2w= k$.
\end{definition}

\begin{remark}
The bounded Gaussian mechanism would not add noise to $w_{ij}=0$. This means the bounded Gaussian mechanism would not modify the presence or absence of an edge in a graph.
\end{remark}

Assume the bounded Gaussian mechanism generates private weights $\Tilde{w}$ and $M_{BG}(w)=\Tilde{w}$. Now we can derive a private reproduction number $\Tilde{R}_0$ using the private graph $\Tilde{G}=(V,E,\Tilde{w})$:
\begin{equation}
    \Tilde{R}_0 = \rho(\Tilde{G}).
\end{equation}

The private reproduction number $\Tilde{R}_0$ satisfies the same level of privacy protection, i.e., $\epsilon$, in Definition~\ref{def:differential_privacy} as the private weights $\Tilde{w}$ since differential privacy is robust to the post-processing~\cite{dwork2014algorithmic}. The accuracy of $\Tilde{R}_0$ is quantified next.

\begin{thm}\label{concentration_bound_input_perturb}
    Let $\alpha_{ij}=\frac{-w_{ij}}{\sigma}$ and $\beta_{ij}=\frac{\Bar{w}-w_{ij}}{\sigma}$. Given a graph $G=(V,E,w)$ with its reproduction number $R_0=\rho(G)$ and a privacy parameter $\epsilon$, for private graphs $\Tilde{G}=(V,E,\Tilde{w})$, whose weights $\Tilde{w}=M_{BG}(w)$, as well as the private reproduction number $\Tilde{R}_0=\rho(\Tilde{G})$,
    \begin{equation}
        \mathbb{E}[|\Tilde{R}_0-R_0|] \leq \sigma \cdot \sqrt{n^2-\sum_{i=1}^n\sum_{j=1}^n\frac{\beta_{ij}\varphi(\beta_{ij})-\alpha_{ij}\varphi(\alpha_{ij})}{\Phi(\beta_{ij})-\Phi(\alpha_{ij})}},
    \end{equation}
    where $\varphi(\cdot)$ and $\Phi(\cdot)$ are the probability density function and the cumulative distribution function of the standard normal distribution respectively.
\end{thm}

\emph{Proof:} See Appendix~\ref{apdx:proof_concentration_bound_input_perturb}.

\bo{It is really hard to say something about this bound. We will explain it in the simulation section.}

\subsection{Output Perturbation Mechanism}

 We start with the sensitivity.
\begin{lemma}[Sensitivity]\label{lem:sensitivity}
    Given any adjacent graphs $G$ and $G'$, the sensitivity of $R_0$, written as $\Delta R$ is defined as
    \begin{equation*}
        \Delta R = \max_{G,G' s.t. \adj_{k}(G,G')=1}|\rho(\Gamma^{-1}B(G))-\rho(\Gamma^{-1}B(G')|\leq k
    \end{equation*}
\end{lemma}
\emph{Proof}: See Appendix~\ref{apdx:proof_sensitivity}.\hfill $\blacksquare$

Because $R_0$ has a bounded support $(0,\bar{R}_0]$, we will use the bounded Laplace mechanism.
\begin{definition}[Bounded Laplace mechanism; Solution to Problem~\ref{prob:privacy_mechanism_design}]\label{def:bounded_laplace}
     Let $b>0$ and let $D=(0,\bar{R}_0]$ be a bounded domain with $l<u$ and both finite. 
	Then the bounded Laplace mechanism $M:\Omega \rightarrow D$, for each
	$R_0\in D$, is given by its probability density function $f$ as
	\begin{equation}
		f(x)
		=\begin{cases}
			0 & \text{if }x\notin D\\
			\frac{1}{C_R(b)}\frac{1}{2b}e^{-\frac{|x-R_0|}{b}} & \text{if }x\in D
		\end{cases},
	\end{equation}
	\noindent where $C_{R}(b)=\int_{D}\frac{1}{2b}e^{-\frac{|x-R_0|}{b}}dx$ is a normalizing
term. And the bounded Laplace machanism $M$ is $(\epsilon,\delta)$-differentially private when 
\begin{equation*}
    b\ge\frac{\Delta R}{\epsilon-\log\Delta C(b)-\log(1-\delta)}.
\end{equation*}\hfill
\end{definition}

We now solve for other parameters in Definition~\ref{def:bounded_laplace}. We first find an explicit formula for $C_R(b)$.
\begin{lemma}[Find $C_R(b)$]
    For $R_0\in D$ where $D=(0,\bar{R}_0]$, and $C_R(b)$ defined in Definition~\ref{def:bounded_laplace}, we have
    \begin{equation}
        C_R(b) = 
        1-\frac{1}{2}\left(\exp\left(-\frac{R_0}{b}\right)-\exp\left(-\frac{\Bar{R_0}-R_0}{b}\right)\right) \label{eq:scaling_parameter}
    \end{equation}
\end{lemma}
\emph{Proof:} By Lemma 3.2 in the bounded Laplace paper, for $R_0\in[l,u]$, we have

\begin{equation*}
    C_R(b) = 1 - \frac{1}{2}\left(e^{-\frac{R_0-l}{b}}+e^{-\frac{u-R_0}{b}}\right)
\end{equation*}

We can plug in $l=0$ and $u=\Bar{R}_0$ then done. \hfill$\blacksquare$

We next give an explicit formula for $\Delta C(b)$. 
\begin{lemma}[Find $\Delta C(b)$]
     For $R_0\in D$ where $D=(0,\bar{R}_0]$, the $\Delta C(b)$ in the Definition~\ref{def:bounded_laplace} is defined as
    \begin{equation*}
        \Delta C(b) =
            \frac{1-\frac{1}{2}\left(\exp\left(-\frac{k}{b}\right)+\exp\left(-\frac{\Bar{R}_0-k}{b}\right)\right)}{1-\frac{1}{2}\left(1+\exp\left(-\frac{\Bar{R}_0}{b}\right)\right)}
    \end{equation*}
\end{lemma}
\emph{Proof:} By Definition 3.4 in the bounded Laplace mechanism paper, for $R_0\in[l,u]$, we have
\begin{equation*}
    \Delta C(b) = \frac{C_{l+\Delta R}(b)}{C_l(b)}
\end{equation*}

We finish the proof by plugging in corresponding $l$ and $\Delta R$.\hfill$\blacksquare$

We now can use Algorithm 1 in the bounded Laplace mechanism paper to find $b$. We now show how accurate $\tilde{R}_0$ is.
\begin{lemma}[Solution to Problem~\ref{prob:accuracy_private_r0}]
    Given bounded Laplace mechanism in Definition~\ref{def:bounded_laplace} with $D=(0,\Bar{R}_0]$, then we have the following bounds:
    \begin{equation*}
       \mathbb{P}(\Tilde{R}_0\in [l,u]) = \frac{1-\frac{1}{2}\left(\exp\left(-\frac{R_0-l}{b}\right)+\exp\left(-\frac{u-R_0}{b}\right)\right)}{C_R(b)},
   \end{equation*}
   where $[l,u]\subset D$.
\end{lemma}
\emph{Proof:} Given a bounded range $[l,u]\subset D$ where $D=(0,\Bar{R}_0]$, we have 
\begin{align}
   \mathbb{P}(\Tilde{R}_0\in[l,u]) &= \int_l^u \frac{1}{C_R(b)}\frac{1}{2b}e^{-\frac{|x-R_0|}{b}}dx\nonumber\\
    &= \frac{1-\frac{1}{2}\left(\exp\left(-\frac{R_0-l}{b}\right)+\exp\left(-\frac{u-R_0}{b}\right)\right)}{C_R(b)}\label{Eq:1} 
\end{align}
where Equation~\eqref{Eq:1} is from Lemma 3.2 in the bounded Laplace mechanism paper and $C_R(b)$ is derived by Equation~\eqref{eq:scaling_parameter}.

==> privacy_mechanism_v2.tex <==
\section{Privacy mechanisms for the reproduction number}\label{sec:results}
In this section, we develop two distinct differentially private mechanisms that enforce differential privacy - one utilizing the input perturbation and the other employing the output perturbation. 

\subsection{Input Perturbation Mechanism}
The input perturbation mechanism provides differential privacy guarantee by generating private values for the weights of a graph. Specifically, we use the bounded Gaussian mechanism~\cite{chen2022bounded} for this purpose. We start by defining the sensitivity, which captures the maximum impact on outputs of changing a weighted graph $G=(V,E,W)$ to \baike{its} adjacent graph $G'=(V,E,W')$ in Definition~\ref{def:adjacency}.   

\begin{definition}[$L_2$ sensitivity]
The $L_2$ sensitivity is defined as:
\begin{equation*}
    \Delta_2 w = \max_{\substack{G, G' \in \mathcal{G}_n \\ ||W-W'||_1 \leq k}} \sqrt{\sum_{i,j}(w_{ij}-w_{ij}')^2},
\end{equation*}
where $k$ is an adjacency parameter with respect to Definition~\ref{def:adjacency}. \hfill $\lozenge$
\end{definition}
Since the $L_2$ sensitivity is defined by $L_2$ norm of the vector-wise entries difference, by the nature of norms we have
\begin{equation}
    \Delta_2 w \leq k.\label{eq:l2_sensitivity_upper_bound}
\end{equation}

We then use this upper bound on $\Delta_2w$ to calibrate the variance of noise needed to protect privacy.

\begin{mechanism}[Bounded Gaussian mechanism; Solution to Problem~\ref{prob:input_perturbation_design}]\label{mech:bounded_Gaussian_mechanism}
Fix a probability space $(\Omega,\mathcal{F},\mathbb{P})$. Let $\sigma>0$ and let $G=(V,E,W)$ be the sensitive graph. Then for $D=(0,\bar{w}]$, the bounded Gaussian mechanism $M_{BG}:D^{n_w}\times \Omega \rightarrow D^{n_w}$ generates independent private weights $\Tilde{w}_{ij}\sim \text{TrunG}(w_{ij},\sigma,0,\Bar{w})$.
%with the probability density function $p_{M_{BG}}$:
%\begin{align}
%    p_{M_{BG}}(\Tilde{w}_{ij}) = \begin{cases}
%        \frac{1}{C_{w_{ij}}(\sigma)} \exp\left(-\frac{(\Tilde{w}_{ij}-w_{ij})^2}{2\sigma^2}\right) & \text{if } \Tilde{w}_{ij}\in D \\
%        0 & \text{otherwise}
%    \end{cases},
%\end{align}
%where $C_{w_{ij}}(\sigma)=\int_D \exp\left(-\frac{(\Tilde{w}_{ij}-w_{ij})^2}{2\sigma^2}\right)d\Tilde{w}_{ij}$ is the normalizing term. 
The minimal $\sigma=\Omega\left(\sqrt{\frac{2\Bar{w}\Delta_2w+(\Delta_2w)^2}{\epsilon}}\right)$ that satisfies $\epsilon$-differential privacy can be found using \cite[Algorithm 2]{chen2022bounded} by setting $\Delta_2w= k$.\hfill $\lozenge$
\end{mechanism}

When the privacy parameter $\epsilon$ increases, the parameter $\sigma$ in the bounded Gaussian mechanism decreases. And when $\epsilon\rightarrow 0$, we have $\sigma\rightarrow\infty$, and $\text{TrunG}(w_{ij},\sigma,0,\Bar{w})$ converges to $\text{Uniform}(0,\Bar{w})$ for all $w_{ij}$. 

\begin{remark}
The bounded Gaussian mechanism would not add noise to $w_{ij}=0$. This means the bounded Gaussian mechanism would not modify the presence or absence of an edge in a graph.
\end{remark}

Assume the bounded Gaussian mechanism generates private weights matrix $\Tilde{W}$ and $M_{BG}(W)=\Tilde{W}$. Now we can derive a private reproduction number $\Tilde{R}_0$ using the private graph $\Tilde{G}=(V,E,\Tilde{W})$:
\begin{equation}
    \Tilde{R}_0 = \rho(\Tilde{W}).
\end{equation}
The private reproduction number $\Tilde{R}_0$ satisfies the same level of privacy protection, i.e., $\epsilon$, in Definition~\ref{def:differential_privacy} as the private weights matrix $\Tilde{W}$ since differential privacy is robust to the post-processing~\cite{dwork2014algorithmic}. The accuracy of $\Tilde{R}_0$ is quantified next.
\baike{[In theorem 1, we didn't define what is a reproduction number of a graph. We need to define this term in the problem formulation section.]}
\begin{thm}\label{thm:expectation_bound_input_perturb}
    Let $\alpha_{ij}=\frac{-w_{ij}}{\sigma}$ and $\beta_{ij}=\frac{\Bar{w}-w_{ij}}{\sigma}$. Given a sensitive graph $G=(V,E,W)$ with its reproduction number $R_0=\rho(W)$, for private graphs $\Tilde{G}=(V,E,\Tilde{W})$, whose weights $\Tilde{W}=M_{BG}(W)$ is generated by the bounded Gaussian mechanism with privacy parameter $\epsilon$ and the private reproduction number $\Tilde{R}_0=\rho(\Tilde{W})$, we have
    \begin{align}
        \mathbb{E}[\Tilde{R}_0-R_0]&\leq\mathbb{E}[|\Tilde{R}_0-R_0|] \\&\leq \sigma \cdot \sqrt{n_w-\sum_{i=1}^n\sum_{j=1}^n\frac{\beta_{ij}\varphi(\beta_{ij})-\alpha_{ij}\varphi(\alpha_{ij})}{\Phi(\beta_{ij})-\Phi(\alpha_{ij})}}\\
        &\leq \sigma\sqrt{n_w},\label{eq:abs_expectation_bounds_input_perturb}
    \end{align}
    and
    \begin{align}
        &\mathbb{E}[(\Tilde{R}_0-R_0)^2]\\
        &\leq \sigma^2\cdot\left(n_w-\sum_{i=1}^n\sum_{j=1}^n\frac{\beta_{ij}\varphi(\beta_{ij})-\alpha_{ij}\varphi(\alpha_{ij})}{\Phi(\beta_{ij})-\Phi(\alpha_{ij})}\right)\\
        &\leq \sigma^2n_w.\label{eq:mse_bounds_input_perturb}
    \end{align}
\end{thm}

\emph{Proof:} See Appendix~\ref{apdx:proof_expectation_bound_input_perturb}.\hfill $\blacksquare$

A larger $\epsilon$ indicates weaker privacy which results in a smaller $\sigma$ and $\mathbb{E}[|\Tilde{R}_0-R_0|]$ closer to $0$. We next state a tail bound on the $\tilde{R}_0$.

\begin{thm}[Tail bounds]\label{thm:input_perturb_tail}
    Given a sensitive graph $G=(V,E,W)\in\mathcal{G}^n$ with its reproduction number $R_0=\rho(W)$, for private graphs $\tilde{G}=(V,E,\tilde{W})\in\mathcal{G}^n$ whose weights $\tilde{W}=M_{BG}(W)$ is generated by the bounded Gaussian mechanism with privacy parameter $\epsilon$ and private reproduction number $\tilde{R}_0=\rho(\tilde{W})$, we have
    \begin{equation}
        \tilde{R}_0 - R_0\leq \sigma\sqrt{n_w} + r,
    \end{equation}
    where $r$ is a random variable that satisfies the tail bound:
    \begin{equation}
        \mathbb{P}[r>t]\leq C\cdot\exp\left(-\frac{t^2}{2\sigma^2}\right),
    \end{equation}
    where $C=2\cdot 9^{2n}$ and $\sigma$ is the minimal value that is required for the bounded Gaussian mechanism to satisfy $\epsilon$-differential privacy.
\end{thm}
\emph{Proof:} See Appendix~\ref{apdx:proof_input_perturb_tail}.\hfill $\blacksquare$


\subsection{Output Perturbation Mechanism}

The output perturbation mechanism is employed to generate differentially private values by first computing the reproduction number $R_0$ on the original graph $G=(V,E,w)$ and subsequently producing a private approximation $\Tilde{R}_0$ based on the computed $R_0$. To achieve this, we use the bounded Laplace mechanism~\cite{holohan2018bounded}. The bounded Laplace mechanism uses $L_1$ sensitivity, which is defined next. \bo{Should we give a reason why not using bounded Gaussian for output perturbation?}
\begin{definition}[$L_1$ sensitivity]\label{def:L1_sensitivity}
    The $L_1$ sensitivity is defined as:
    \begin{equation}
        \Delta_1\rho = \max_{\substack{G, G' \in \mathcal{G}^n \\ ||W-W'||_1 \leq k}} |\rho(W)-\rho(W')|,
    \end{equation}
    where $k$ is an adjacency parameter with respect to Definition~\ref{def:adjacency}. \hfill $\lozenge$
\end{definition}

The following lemma provides a bound on the sensitivity defined in Definition~\ref{def:L1_sensitivity}.

\begin{lemma}\label{lem:sensitivity}
    Given an adjacency parameter $k$ with respect to Definition~\ref{def:adjacency}, the $\Delta_1\rho$ in Definition~\ref{def:L1_sensitivity} satisfies
    \begin{equation}
        \Delta_1\rho \leq k.
    \end{equation}
\end{lemma}
\emph{Proof}: See Appendix~\ref{apdx:proof_sensitivity}.\hfill $\blacksquare$

Next, we will introduce the bounded Laplace mechanism. Since $R_0$ lies within the interval $D_R=(0,\bar{R}_0]$, the bounded Laplace mechanism will ensure that the generated private values are restricted to this range.
\begin{mechanism}[Bounded Laplace mechanism; Solution to Problem~\ref{prob:output_perturbation_design}]\label{mech:bounded_laplace}
     Fix a probability space $(\Omega,\mathcal{F},\mathbb{P})$. Let $b>0$ and let $G=(V,E,W)$ be the sensitive graph.
	For $D_R=(0,\bar{R}_0]$, the bounded Laplace mechanism $M_{BL}:D_R\times\Omega \rightarrow D_R$ generates private values $\Tilde{R}_0\sim\text{TrunL}(R_0,b,0,\Bar{R}_0)$. The minimal $b=\Omega\left(\frac{\Delta_1\rho}{\epsilon}\right)$ that satisfies $\epsilon$-differential privacy can be found using~\cite[Algorithm 1]{holohan2018bounded} by setting $\Delta_1\rho=k$.\hfill $\lozenge$
\end{mechanism}

The accuracy of $\Tilde{R}_0$ generated by the bounded Laplace mechanism can be quantified using the next Lemma.

\begin{thm}\label{thm:expectation_bound_output_perturb}
    Let $u=-\frac{\Bar{R}_0-R_0}{b}$ and $l=-\frac{R_0}{b}$. Given a graph $G=(V,E,W)$ with its reproduction number $R_0=\rho(W)$ and a privacy parameter $\epsilon$, the private reproduction number $\Tilde{R}_0$ generated by Mechanism~\ref{mech:bounded_laplace} satisfies
    \begin{align}
        \mathbb{E}[|\Tilde{R}_0-R_0|] = \frac{b(2+(l-1)\exp(l)+(u-1)\exp(u))}{2C(R_0,b)},
    \end{align}
    and
    \begin{align}
        \mathbb{E}[(\Tilde{R}_0-R_0)^2]&=\frac{b^2\left(\gamma_{low}\left(3,-l\right)-\gamma_{low}\left(3,-u\right)\right)}{2C(R_0,b)}\\
        &\leq 2b^2.\label{eq:mse_bounds_output_perturb}
    \end{align}
\end{thm}
\emph{Proof:} See Appendix~\ref{apdx:proof_expectation_bound_output_perturb}.\hfill $\blacksquare$

%\subsection{Comparison between Input and Output Perturbation Mechanisms}

%\subsubsection{High Privacy Regime}
%We start by comparing the input and output perturbation mechanisms in the regime $\epsilon\rightarrow 0$, i.e, both $\sigma\rightarrow 0$ and $b\rightarrow 0$. Therefore for the output perturbation we have $\Tilde{R}_0\sim Uniform(0,n\bar{w})$. As for the input perturbation we have the private weights $\Tilde{w}\sim Uniform(0,\bar{w})$. Applying Theorem~\ref{}, we have 
%\begin{equation}
%    \rho(\tilde{G})\leq ||\Tilde{w}||_2\leq\sqrt{\sum_{e\in E}w(e)}\leq \sqrt{n_e}\bar{w}\leq n\bar{w}.
%\end{equation}

%As a result, the private spectral radius using the input perturbation has a shorter bounded support comparing the one generated by the output perturbation. 

%\subsubsection{Low Privacy Regime}
%For the input perturbation, by combining Mechanism~\ref{mech:bounded_Gaussian_mechanism}, Theorem~\ref{thm:expectation_bound_input_perturb}, and Equation~\eqref{eq:l2_sensitivity_upper_bound}, we have
%\begin{align}
%    E[(\Tilde{R}_0-R_0)^2]&\leq \Theta\left(\frac{n_w(2\Bar{w}\Delta_2w+(\Delta_2w)^2)}{\epsilon}\right)\\
%    &\leq \Theta\left(\frac{n_w(2\Bar{w}k+k^2)}{\epsilon}\right).\label{eq:input_perturb_var_upper_bound_low_privacy}
%\end{align}

%While for the Output perturbation, we can combine Mechanism~\ref{mech:bounded_laplace}, Theorem~\ref{thm:expectation_bound_output_perturb}, and Lemma~\ref{lem:sensitivity} to get
%\begin{align}
%    E[(\Tilde{R}_0-R_0)^2] &\leq \Theta\left(\frac{2(\Delta_1\rho)^2}{\epsilon^2}\right)\\
%    &\leq \Theta\left(\frac{2k^2}{\epsilon^2}\right).
%\end{align}

%With $\epsilon>>1$, Equation~\eqref{eq:input_perturb_var_upper_bound_low_privacy} states the spread of random variable $\tilde{R}_0-R_0$ decays 

